Efficient Interactive Coding Achieving Optimal Error Resilience Over the Binary Channel

Given a noiseless protocol $\pi_0$ computing a function $f(x, y)$ of Alice and Bob's private inputs $x, y$, the goal of interactive coding is to construct an error-resilient protocol $\pi$ computing $f$ such that even if some fraction of the communication is adversarially corrupted, both parties still learn $f(x, y)$. Ideally, the resulting scheme $\pi$ should be positive rate, computationally efficient, and achieve optimal error resilience. While interactive coding over large alphabets is well understood, the situation over the binary alphabet has remained evasive. At the present moment, the known schemes over the binary alphabet that achieve a higher error resilience than a trivial adaptation of large alphabet schemes are either still suboptimally error resilient [EKS20], or optimally error resilient with exponential communication complexity [GZ22]. In this work, we construct a scheme achieving optimality in all three parameters: our protocol is positive rate, computationally efficient, and resilient to the optimal $\frac16 - \epsilon$ adversarial errors. Our protocol employs a new type of code that we call a layered code, which may be of independent interest. Like a tree code, a layered code allows the coder to encode a message in an online fashion, but is defined on a graph instead of a tree.

==> 1.6/old-protocol.tex <==
\subsection{Formal Protocol}
We are now ready to formally state the protocol.

Let $\tc_\epsilon$ be an $\epsilon$-list tree code from $\{00, 01,10,11,\rewind,\bullet\} \to [k]$, for some $k=k(\epsilon)$. When $\epsilon$ is clear, we simply denote it $\tc$. The decoding function of $\tc$ will be $\tcdec$.

Also, $\ECC$ will denote the error correcting code $\ECC_{\epsilon,k}$ as defined in Definition~\ref{def:ecc} when $k$ and $\epsilon$ are clear; its length is $M=M(k)$.
\mnote{no confidence counters}
\protocol{Randomized Protocol Resilient to $\frac16 - ?\epsilon$ Corruptions}{1/6}{
    Fix $n \in \bbN, \epsilon>0$. Suppose Alice and Bob's private inputs are $x, y \in \{ 0, 1 \}^n$ respectively, and the shortest protocol computing $f(x,y)$ has transcript $T(x,y)$, abbreviated $T$. We will assume $T$ is alternating and even length. The protocol consists of $K = \frac{T}{\epsilon}$ messages numbered $1, \dots, K$, each of length $k(\epsilon)$. Alice sends the odd messages and Bob sends the even.
    
    \vspace{0.075in}
    
    Alice and Bob track a private guess for the transcript, denoted $T_A \in \{ 0, 1, \rewind, \bullet \}^*$ and $T_B \in \{ 0, 1, \rewind, \bullet \}^*$ respectively. $T_A$ is initialized to $1$ and $T_B$ to $\emptyset$ at the beginning of the protocol. She tracks the question and answer so far as $T^q_A, T^a_A\in ([k]\cup \bullet)^*$ as well. She finally tracks $(z^q_A,z^a_A)\in ([k]\cup \bullet)\times ([k]\cup \bullet)$ as the ``expected next message'' from Bob.
    
    \vspace{0.075in}
    
    In what follows, we describe Alice's behavior. Bob's behavior is identical, except replacing notationally switching $x$ and $y$ and $A$ and $B$ in general. At the end of the protocol, Alice and Bob will output $T_A$ and $T_B$ respectively.
    
    \begin{center}
    {\bf \fbox{Alice}}
    \end{center}
        Alice has just received a message $m$ from Bob. \mnote{whenever we say Alice appends $\delta$ to $T_A$, she also adds her answer $?$ if $0,1$.}
        
        \begin{caseofb}
        \caseb{For some $\delta\in\{0,1,\rewind\}$, we have $d_m(z^q_A,z^a_A,\delta) < \frac13$.}{
            Let $p=1-3d_m(z^q_A,z^a_A,\delta)$.
            \begin{itemize}
               \item With probability $p$, Alice sets $T_A\gets T_A||\delta ?$ and $T^q_A\gets T^q_A||z^q_A$ and $T^a_A\gets T^a_A||z^a_A$. Else (with probability $1-p$), she sets $T_A\gets T_A||\bullet$ and $T^q_A\gets T^q_A||\perp$ and $T^a_A\gets T^a_A||\perp$.
               \item Alice sends $\ECC(\tc(T_A)[-1],\perp,\perp)$. She sets $z^a_A=\tc(T_A)[-1]$ and $z^q_A=\perp$.
            \end{itemize}
        }
        \caseb{$d_m(z^q_A,z^a_A,\perp) < \frac13$.
        \footnote{Note that usually receiving $\perp$ in the last coordinate means Alice did not receive an answer to her question; this is the exception.}}{
            Let $p=1-3d_m(z^q_A,z^a_A,\perp)$.
            \begin{itemize}
                \item With probability $p$, Alice sets $T_A\gets T_A||1?$ and $T^q_A\gets T^q_A||z^q_A$ and $T^a_A\gets T^a_A||z^a_A$. Else (with probability $1-p$), she sets $T_A\gets T_A||\bullet$ and $T^q_A\gets T^q_A||\perp$ and $T^a_A\gets T^a_A||\perp$.
                \item If $z^a_A\neq \perp$, Alice sends $\ECC(\tc(T_A)[-1],\perp,\perp)$. She sets $z^a_A=\tc(T_A)[-1]$ and $z^q_A=\perp$.
                Else she sends $\ECC(\perp,z^q_A\perp)$. She sets $z^a_A=\perp$ and $z^q_A=\tc(\tcdec(T^q_A)||11)[-1]$ (if $\tcdec=\emptyset$, then she sends $\ECC(\perp,\perp,\perp)$ and sets $z^a_A=\emptyset$ and $z^q_A=\emptyset$).
            \end{itemize}
        }
        \caseb{Not the above, and for some $(q^*,a^*,\perp)$, we have $d_m(q^*,a^*,\perp) \le \frac16$, and not $q^*=a^*=\perp$.} {
            Let $T'=\tcdec(T^q_A||q^*)$ if $q^*\neq \perp$, else let $T'=\tcdec(T^a_A||a^*)$. 
            \begin{subcaseofb}
                \subcaseb{$T'$ amounts to a transcript of length $\geq |T|$ that Alice cannot contradict based on $x$ (note: not based on her guess $T_A$.) }{
                    Let $p=0.5-3d_m(q^*,a^*,\perp)$.
                    \begin{itemize}
                        \item With probability $p$, Alice sets $T^q_A\gets T^q_A||q^*$ and $T^a_A\gets T^a_A||a^*$. She then updates (sets $T_A$) based on $T'$. \mnote{might need to update based on $T^a_A$ if $q^*=\perp$. Also might need to factor in $\delta$?}. Else, with probability $1-p$, she sets $T^q_A\gets T^q_A||\perp$ and $T^a_A\gets T^a_A||\perp$.
                        \item If $q^*\neq \perp$ and Alice's current transcript $T_A$ is $T'$, Alice sends $\ECC(\perp,q^*,\perp)$. She sets $z^a_A=\perp$ and $z^q_A=\tc(\tcdec(T^q_A)||11)[-1]$ (if $\tcdec=\emptyset$, then she sends $\ECC(\perp,\perp,\perp)$ and sets $z^a_A=\emptyset$ and $z^q_A=\emptyset$). Else, Alice sends $\ECC(\tc(T_A)[-1],\perp,\perp)$. She sets $z^a_A=\tc(T_A)[-1]$ and $z^q_A=\perp$.
                    \end{itemize}
                }
                \subcaseb{Not the above.}{
                    Let $p=1-6d_m(q^*,a^*,\perp)$.
                    \begin{itemize}
                        \item Alice sets $T_A\gets T_A||\bullet$. With probability $p$, she sets $T^q_A\gets T^q_A||q^*$ and $T^a_A\gets T^a_A||a^*$. Else, she sets $T^q_A\gets T^q_A||\perp$ and $T^a_A\gets T^a_A||\perp$.
                        \item If she rolled probability $p$ above: if $q^*\neq \perp$, she computes an answer $a$ to $T^q_A$ and sends $\ECC(\perp,q^*,a)$; else she computes an answer $a$ to $T^a_A$ and sends $\ECC(\tc(T^a_A||1)[-1],\perp,a)$. She sets $z^a_A=\emptyset$ and $z^q_A=\emptyset$. Else, she sends $\ECC(\tc(T_A)[-1],\perp,\perp)$. She sets $z^a_A=\tc(T_A)[-1]$ and $z^q_A=\perp$.
                    \end{itemize}
                    
                }
            \end{subcaseofb}
        }
        \caseb{None of the above.}{
            \begin{itemize}
                \item Alice sets $T_A\gets T_A||\bullet$ and $T^q_A\gets T^q_A||\perp$ and $T^a_A\gets T^a_A||\perp$.
                \item Alice sends $\ECC(\tc(T_A)[-1],\perp,\perp)$. She sets $z^a_A=\tc(T_A)[-1]$ and $z^q_A=\perp$.
            \end{itemize}
        }
        
        \end{caseof}
        
}

==> 1.6/treecodes.tex <==
\subsection{Tree Code Preliminaries}

\begin{definition}[Tree Code]
A tree code $\tc : \Sigma_{in} \to \Sigma_{out}$ is a code such that $\tc(x)_i$ depends only on
$x[1, . . . , i]$. We will also write $C(x) \in \Sigma^i_{out}$ for $i < n$, $x \in \Sigma^i_{in}$.
\end{definition}

\begin{definition}[Suffix Distance]

\end{definition}

We will need something stronger than a tree code; we define a list tree code for this. Note that our definition is slightly different, but quite similar to the ones in \cite{Gelles-survey} and \cite{BravermanE14}.

\begin{definition}[$L_i$]
For any tree code $\tc$, any $\epsilon$, and word $w$ of length $n$, let the list $L_i(\tc,w,\epsilon)$ be the list of codewords $x$ of length $i$ that are close to a prefix of length $i$ of $w$ in their suffix
distance, that is,

$$L_i(\tc,w,\epsilon) = \{x_1 · · · x_i
: \Delta_{sfx}(\tc(x_1 · · · x_i), w_1 · · · w_i) < 1-\epsilon\}.$$ 

When $\tc$ and $w$ and $\epsilon$ are clear, we will often abbreviate $L_i(\tc,w,\epsilon)$ as $L_i$.

$L=\bigcup_{i=1}^{n} L_i$.
\end{definition}

\begin{definition}[List Tree code]
A tree code $\tc : \Sigma_{in} \to \Sigma_{out}$ is a $\epsilon$-list tree code if it additionally satisfies the following property. 

For any word $w$ of length $n$, for at least $(1-\epsilon)n$ values of $i<n$, we have $|L_i|\leq 1$.
\end{definition}

\begin{definition}[$\tcdec$]
Given an $\epsilon$-list tree code, the function $\tcdec(w) : \Sigma_{out}\to \Sigma_{in}$ returns $x$ such that $\Delta(\tc(x),w)\leq (1-\epsilon)$. Returns $\emptyset$ if there are $0$ or multiple such $x$.
\end{definition}

\begin{theorem}[List Tree Codes Exist]\label{thm:list-tree}
For every $\epsilon$, there exists an $\epsilon$-list tree code.
\end{theorem}

The proof follows directly from Theorem 22 in \cite{BravermanE14}, but we will need to define prefix lists to state their theorem and prove ours.

\begin{definition}[$PL$]
Let the prefix list $$PL(\tc, w, \epsilon) := \{y \in \Sigma^*_{in} : y = x[1, . . . , k]\}$$ for some $k$ and some $x \in L(\tc, w, \epsilon)$.

Again, we abbreviate $PL(\tc, w, \epsilon)$ as $PL$.
\end{definition}

\begin{theorem}\cite{BravermanE14}
For every $\epsilon, \Sigma_{in}$, there exists a tree code $\tc: \Sigma_{in}\to \Sigma_{out}$ where $|\Sigma_{out}|=O_\epsilon(\Sigma_{in})$ such that the following holds. For any $w$ of length $n$, we have that for $\leq (1+\epsilon)n$ values of $x\in PL$, we have $\tc(x)[|x|]=w[|x|]$.
\end{theorem}

We return to the proof of Theorem~\ref{thm:list-tree}.

\begin{proof}
For any $w$, define $w'$ as follows. Let $$PL_i(w)=\{x : x\in PL(w), |x|=i\}.$$ If for all $x\in PL_i(w)$, we have $x[i]\neq w[i]$, then let $w'[i]=x[i]$ for any arbitrary $x\in PL_i(w)$. Otherwise let $w'[i]=w[i]$.

Notice that for all $i$, we have $L_i(w)\subseteq L_i(w')$ because for all changed indices $i$, no element $x\in L(w)$ has $x[i]=w[i]$, so the distance to any prefix of $w$ cannot increase. This implies $PL(w)\subseteq PL(w')$ as well. Then, we always have that for at least one $x\in PL_i(w')$, we have $w'[i]=x[i]$. Since the total number of $x\in PL_i(w')$ summed over all $i$ such that $w'[|x|]=x[|x|]$ is $\leq (1+\epsilon)n$, only on $\epsilon$ indices can this value be at least $2$ (in other words more than $1$. Thus, for $(1-\epsilon)$ indices $i$, the number of $x\in PL_i(w')$ such that $x[i]=w'[i]$ is $\leq 1$. 

Finally, notice that $L_i(w')\subseteq \{x : x\in PL_i(w'), x[i]=w'[i]\}$, and so $$|L_i(w')|\leq 1\implies |L_i(w)\leq 1$$ since $L_i(w)\subseteq L_i(w')$.
\end{proof}

We state another important lemma -- the proof appears in \cite{Gelles-survey}.

\begin{lemma} [\cite{Gelles-survey}]\label{lem:dec-freq}
For any $r, s \in \Sigma^n$, if $\Delta(r, s) = \beta n$, then there exists a set of indices $I \subseteq [n]$ of size
$|I| \ge (1 - \beta/\alpha)n$ such that for any $i \in I$,
$$ \Delta_{sfx}(r_1, \dots, r_i
, s_1, \dots, s_i) < \alpha.$$
\end{lemma}

Another useful theorem is the following:

\begin{theorem}\label{thm:treecodes}
For every $\epsilon, n$, for any $\epsilon$-list tree code $\tc:\Sigma_{in}^n\to \Sigma_{out}^n$ such that for any $x\in \Sigma_{in}$, for any $w\in \Sigma_{out}$, let $I$ be the set of indices where $\tc(x)[i]=w[i]$. For all but $5\epsilon n$ values of $i\in I$, we have $\tcdec(w[:i])=x[:i]$.
\end{theorem}

\begin{proof}
Follows from Lemma~\ref{lem:dec-freq}.

For an $\epsilon$-tree code, there is at most one list tree code option other than $\epsilon n$ of the time. By Lemma~\ref{lem:dec-freq}, there is one option correct at least $n(1-\frac{1}{1-\epsilon})-|I|/(1-\epsilon)>-2\epsilon n-|I|-2\epsilon|I|$\mnote{Uses $\epsilon<0.5$.} of the time. Subtracting off the times there are multiple options, we get $|I| - 5\epsilon n$ times.
\end{proof}
